Practical Prescribed-Time Seeking of a Repulsive Source by Unicycle Angular Velocity Tuning

All the existing source-seeking algorithms for unicycle models in GPS-denied settings guarantee at best an exponential rate of convergence over an infinite interval. Using the recently introduced time-varying feedback tools for prescribed-time stabilization, we achieve source seeking in prescribed time, i.e., the convergence to a small but bounded neighborhood of the source, without the measurements of the position and velocity of the unicycle, in as short a time as the user desires, starting from an arbitrary distance from the source. The practical convergence is established using a singularly perturbed version of the Lie bracket averaging method, combined with time dilation and time contraction operations. The algorithm is robust, provably, even to bounded nonvanishing perturbations and an arbitrarily strong gradient-dependent repulsive velocity drift emanating from the source.

==> Paper tex file - Arxiv sub/plots/stable_F.tex <==
\begin{tikzpicture}
		\begin{axis}[
		width = 7.8cm,
		height = 5cm,
		xmin = 0,
		xmax = 3.5,
		ylabel={$F(x)$},
		xlabel={$t$},
		grid=major]
		\addplot [very thick,red] table[x = t, y = y]{plots/stable_F_exp.dat};
		\addplot [thick,blue] table[x=tpt, y = ypt]{plots/stable_F_PT.dat};
		\end{axis};	
\end{tikzpicture} 

	

==> Paper tex file - Arxiv sub/plots/unstable_F.tex <==
\begin{tikzpicture}
		\begin{axis}[
		width = 7.8cm,
		height = 5cm,
		xmin = 0,
		xmax = 2.5,
		ylabel={$F(x)$},
		xlabel={$t$},
		grid=major]
		\addplot [very thick,red] table[x = t, y = y]{plots/unstable_F_exp.dat};
		\addplot [thick,blue] table[x = tpt, y = ypt]{plots/unstable_F_PT.dat};
		\end{axis};	
\end{tikzpicture} 

	

==> plots/stable_F.tex <==
\begin{tikzpicture}
		\begin{axis}[
		width = 7.8cm,
		height = 5cm,
		xmin = 0,
		xmax = 3.5,
		ylabel={$F(x)$},
		xlabel={$t$},
		grid=major]
		\addplot [very thick,red] table[x = t, y = y]{plots/stable_F_exp.dat};
		\addplot [thick,blue] table[x=tpt, y = ypt]{plots/stable_F_PT.dat};
		\end{axis};	
\end{tikzpicture} 

	

==> plots/unstable_F.tex <==
\begin{tikzpicture}
		\begin{axis}[
		width = 7.8cm,
		height = 5cm,
		xmin = 0,
		xmax = 2.5,
		ylabel={$F(x)$},
		xlabel={$t$},
		grid=major]
		\addplot [very thick,red] table[x = t, y = y]{plots/unstable_F_exp.dat};
		\addplot [thick,blue] table[x = tpt, y = ypt]{plots/unstable_F_PT.dat};
		\end{axis};	
\end{tikzpicture} 

	
